Network Inference by Learned Node-Specific Degree Prior

We propose a novel method for network inference from partially observed edges using a node-specific degree prior. The degree prior is derived from observed edges in the network to be inferred, and its hyper-parameters are determined by cross validation. Then we formulate network inference as a matrix completion problem regularized by our degree prior. Our theoretical analysis indicates that this prior favors a network following the learned degree distribution, and may lead to improved network recovery error bound than previous work. Experimental results on both simulated and real biological networks demonstrate the superior performance of our method in various settings.

==> llpdfus1 <==
#!/bin/bash

# PDF with lossless compression and font embedding. This also embeds fonts
# inside Matlab figures.
# Ghostscript will *not* embed the base 14 fonts (Times, Helvetica, etc.)
# under PDF level 1.2, so use CompatibilityLevel=1.3.

ps2pdf -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode \
       -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode \
       -dEmbedAllFonts=true -dMaxSubsetPct=100 -dSubsetFonts=true \
       -sPAPERSIZE=letter -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress $1

# The lossless compression can also be achieved by adding the options
# inside the LaTeX source with the following \special (and then running
# ps2pdf without the options):
# 
# \AtBeginDvi{\special{!
#   /setdistillerparams where {pop}{userdict /setdistillerparams {pop} put}ifelse
#   <<
#   /AutoFilterColorImages false
#   /AutoFilterGrayImages false
#   /ColorImageFilter /FlateEncode
#   /GrayImageFilter /FlateEncode
#   >>
#   setdistillerparams
# }}


